On the needs for MaaS platforms to handle competition in ridesharing mobility

Ridesharing has been emerging as a new type of mobility. However, the early promises of ridesharing for alleviating congestion in cities may be undermined by a number of challenges, including the growing number of proposed services and the subsequent increasing number of vehicles, as a natural consequence of competition. In this work, we present optimization-based approaches to model cooperation and competition between multiple ridesharing companies, in a real-time on-demand setting. A recent trend relies on solving the integrated combination of Dial-A-Ride Problems (DARP), which compute the cost of assigning incoming requests to vehicle routes, plus Linear Assignment Problems (LAP), which assign vehicles to requests. While the DARPs, are solved at the level of the vehicles of each company, we introduce cooperative and competitive approaches to solve the LAP. The cooperative model, which could make use of Mobility as a Service platforms, is shown to solve the LAP to optimality following closely results from the literature, and limiting the amount of information the companies are required to share. We investigate how a realistic model of competition deviates from this optimality and provide worst case bounds. We evaluate these models with respect to a centralized model on one-week instances of the New York City taxi dataset. Model variants coping with noise in the travel time estimations, bias in the assignment costs, and preferences in the competitive case are also presented and validated. The computational results suggest that cooperation among ridesharing companies can be conducted in such a way to limit the degradation of the level of service with respect to a centralized model. Finally, we argue that the competition can lower the quality of the ridesharing service, especially in the case customer preferences are accommodated.

==> Assignment.tex <==
% !TEX root = Multi-company_v1.tex

\section{The auction algorithm}	
\label{sec:assignment}

\Cmm{When revising this and next section, please refer to the revised Section 2 for nomenclature. }

%\subsection{General form of the assignment problem}
%
%We formalize here the linear assignment problem (both the initial and the rebalancing one). Let $\mathcal{M}$ denote a set of customer trip requests at time $t$ and $\mathcal{P}$ denote a set of competing companies. For a given batch of requests, each company $p \in \mathcal{P}$ has a fleet of available vehicles, denoted by set $\mathcal{C}_p$, which are available for the customers to request. $\mathcal{C}$ denotes the set of all available vehicles, $\mathcal{C} = \bigcup_{p} \mathcal{C}_p$. Let $p_i$ denote the company to which a vehicle $i \in \mathcal{C}$ belongs. Let $x_{ij} \in \{ 0,1\}, i \in \mathcal{C}, j \in \mathcal{M}$ be the set of binary variables: $x_{ij}=1$ only if vehicle $i$ is assigned to customer $j$, otherwise $x_{ij}=0$. We denote by $j_i$ the customer $j \in \mathcal{M}$ assigned to a vehicle $i \in \mathcal{C}$, that is, $x_{i,j_i}=1$. Let $c_{ij} \in \mathbb{R}_+$ denote the cost incurred by the vehicle if it is assigned to customer $j$. Let $\mathcal{I} : \mathcal{C} \times \mathcal{M} \rightarrow \mathbb{R}_+$ denote the cost function, where $\mathcal{I}(i,j)=c_{ij}$. We set $\mathcal{I}(i,j)= \infty$ if a vehicle $i$ cannot accommodate the request for customer $j$. This cost is typically defined as the travel distance or travel time, considering the different vehicle and customer parameters including detour time required to add the new customer to the current schedule, vehicle capacity, preference of customers already on-board, etc.
%
%
%For our optimization structure, we seek to assign each customer request to available vehicles in each time step such that vehicles are assigned to one and one only new customer. (Vehicles can be assigned to multiple customers over successive time steps, but never within the time step). This yields the following linear assignment problem: 
	%\begin{subequations}
 		%\begin{align}
	 		%\min_{x_{ij} \in \{ 0,1 \}, i\in \mathcal{C}, j \in \mathcal{M} } & \sum_{i=1}^n \sum_{j=1}^m c_{ij} x_{ij} & \label{eq:optimization} \quad \left[  \textbf{LAP(}C,\mathcal{M} \textbf{)} \right]\\
	 		%\text{subject to: } & \sum_{i=1}^n x_{ij} = 1, & j \in \mathcal{M} \label{eq:const1}\\
	 		 %& \sum_{j=1}^m x_{ij} = 1, & i \in \mathcal{C} \label{eq:const2} \\
	 		 %& c_{ij} = \mathcal{I}(i,j), & i \in \mathcal{C}, j \in \mathcal{M}, \label{eq:const3}
 		%\end{align}
 	%\end{subequations}
%where, without loss of generality, we have assumed that the number of vehicles is equal to the number of new customers, $n=m$. Note that if this is not the case, one can augment the problem with dummy vehicles or customers with infinite costs. 
%
%The aim of the optimization is to minimize the total assignment costs \eqref{eq:optimization}: in our implementation, $c_{ij}$ is expressed as the time duration (or TD) of the route of vehicle $i$ that serves the already scheduled customers and the new customer $j$.
%
%\Cmm{Rephrase here, maybe add something that Claudio has written already}
%
 %\paragraph{Solution Method.} Provided that all the costs $c_{ij}$ are precomputed, then (\ref{eq:optimization}-\ref{eq:const3}) can be casted as an asymmetric, or rectangular, LAP \citep{KenH80, PapS82, bijsterbosch2010solving}. It is well known that LAPs have a totally unimodular constraint matrix, hence their continuous relaxation (i.e., substitute $x_{ij}\in\{0,1\}$ with $x_{ij}\in[0,1]$) is exact. We exploit the available efficient solution algorithms for LAPs, in particular the auction algorithm (scaling up to $10^6$ requests), see e.g.~\citep{Bernard2016, bertsekas1990auction}.

%\subsection{The auction algorithm}
%For the auction algorithm, we study a variant of the assignment problem where the objective is changed from minimization to maximization. Define $r_{ij} = -c_{ij}, i\in \mathcal{C}, j \in \mathcal{M}$, as the reward/benefit obtained by vehicle $i$ if customer $j$ is assigned to the vehicle. The objective of the optimization problem changes to $\max_{x_{ij} \in \{ 0,1 \}, i\in \mathcal{C}, j \in \mathcal{M} } \sum_{i=1}^n \sum_{j=1}^m r_{ij} x_{ij}$, subject to the constraints \eqref{eq:const1}--\eqref{eq:const3} and an additional constraint, $r_{ij} = -c_{ij}$.

\Cmm{in this section we present generic results for centralised and distributed auctions algorithms for the case of bidders $\in\mathcal{B}$ and objects $\in\mathcal{O}$. Then conclude that we may apply this to ridesharing settings. This section should be about presenting existing results from the literature, e.g. in the form of Lemmas, and be less verbal.}

In this section we present a general structure of the auction algorithm and the standard results from the literature. Let $x \in X$ be a set of persons to be assigned to the set of objects $y \in Y$. We assume the problem to be symmetric, that is $|X|=|Y|=n$. There is a benefit $a_{xy}$ in assigning person $x$ to object $y$ and we seek to find an assignment that maximizes the total benefit. We know a set $\mathcal{A}$ of pairs $(x,y)$ that can be matched. For each person $x$, denote by $A(x)$ the set of objects that can be matched with $x$, and for each object $y$, denote by $\bar{A}(y)$ a set of persons that can be matched with $y$. We seek an optimal feasible assignment defined as a set of person-object pairs $(1,y_1), (2,y_2), \ldots, (n, y_n)$ from $\mathcal{A}$, such that the objects $y_1, y_2, \ldots, y_n$ are all distinct, and such that the total benefit $\sum_{x=1}^n a_{xy_x}$ is maximized.

Let $\rho_y$ be the price of object $y$ that any person assigned to the object must pay to be assigned to the object. Then, the net value of object $y$ for person $x$ is $a_{xy}-\rho_y$. Logically, each person $x$ would want to be assigned to an object $y_x$ with maximal value, that is,
	\begin{equation}
		a_{xy_x}-\rho_{y_x} = \max_{y \in A(x)} a_{xy}-\rho_y
	\end{equation}

The equilibrium of this economic system is attained when no person has any incentive to act unilaterally for seeking another object. Following result from \cite{bertsekas1990auction} establishes a relationship of this equilibrium with the optimal assignment.

\begin{lemma}
	An assignment and a set of prices that are at equilibrium, maximize the total benefit and are thus optimal
\end{lemma}

The naive-auction algorithms in \cite{bertsekas1990auction} is an intuitive method for solving this equilibrium in an iterative manner. It borrows the structure from standard auctions where unassigned bidders place simultaneous bids on objects and raise the bids iteratively to win the ``best'' object. The algorithm consists of two phases, the bidding phase and the assignment phase. In the bidding phase, each unassigned bidder raises the bid on the most profitable object by the difference between the profit of the most and second-most profitable objects. In the assignment phase, each object is assigned to the highest bidder. The process continues until all bidders are assigned to an object.

The naive-auction algorithm faces an issue when several persons contest a small number of objects that are equally desirable and thus do not raise their prices leading to an never ending cycle. This problem is circumvented by defining a perturbation mechanism to converge to an almost equilibrium, see e.g.~\cite{bertsekas1990auction}. This almost equilibrium is achieved when the value for person $x$ to be assigned to object $y$ is within a constant $\epsilon>0$ of being the maximum, i.e. when:

\begin{equation}
	a_{x y_x} - \rho_{y_x} \geq \max_{y \in A(x)} \{ a_{xy}-\rho_y \} - \epsilon \quad \forall x
\end{equation}

This is called the $\epsilon-$complementary slackness condition ($\epsilon-$CS). The auction algorithm solves for this almost equilibrium. It has the same structure as the naive-auction algorithm, except that in each iteration each person raises the bids on the most profitable object by the difference between the profit of the most and second-most profitable objects plus $\epsilon.$ Following results hold true for the auction algorithm.

\begin{lemma}
	A feasible assignment along with a price vector which satisfies the $\epsilon-$CS condition is within $n\epsilon$ of the optimal
	\label{lem:eCSoptimal}
\end{lemma}

\begin{lemma}
	The running time of the auction algorithm is $O(n^2 \max_{(x,y)} |a_{xy}|/\epsilon)$
\end{lemma}

The auction algorithm lends itself to be easily solved in a distributed or parallel fashion \cite{bertsekas1990auction}. Zavlanos et al. \citep{zavlanos2008distributed} show that if the information of bid prices is shared between ``neighboring" persons, then a distributed version of the auction algorithm which updates the bid prices and assignment of each person based on the bid prices and previous assignment of its neighbors can solve for system optimal even under restricted communication between persons. Naparstek and Leshem \cite{naparstek2014fully} present an alternate distributed implementation of the auction algorithm. In their structure, each person maintains an estimate $\hat{B}(x,y)$ of the highest price $\rho_y$ for each object and in each iteration, determines its bid prices based on that estimate. The estimate maintained by each person is different and is updated only when a person wins the bid on a certain object. Since each person does not have access to the true price of an object, the $\epsilon-$CS condition is replaced by a local condition called L$\epsilon-$CS condition, defined as the following:

\begin{equation}
	a_{x y_x} - \hat{B}(x, y_x) \geq \max_{y \in A(x)} \{ a_{xy}- \hat{B}(x, y) \} - \epsilon \quad \forall x
	\label{eq:epsilonCS}
\end{equation}

Following statements is shown to be true

\begin{lemma}
	Given a feasible assignment and a bidding matrix which satisfies the L$\epsilon-$CS condition for all persons, then the $\epsilon-$CS condition is also satisfied for all persons and the assignment is within $n\epsilon$ of the optimal.
\end{lemma}

%The proofs in \cite{naparstek2014fully} show that the distributed implementation terminates and converge to an assignment with costs within $|\mathcal{C}|\epsilon$ of the optimal costs.
%
%The auction algorithm requires 

%Let $\hat{B}(i,j)$ be the bid placed by vehicle $i \in \mathcal{C}$ for customer $j \in \mathcal{M}$. The auction algorithm requires the introduction of a perturbation mechanism to converge to a almost equilibrium, see e.g.~\cite{bertsekas1990auction}. This almost equilibrium is achieved when %at a time $t$ 
%the cost for vehicle $i$ to be assigned to customer $j$ %, i.e. we have $x^*_{ij}=1$, 
%is within a constant $\epsilon>0$ of being minimal, i.e. when:
%	\begin{equation}
%		-c_{ij} - \rho_{j} \geq \max_{1\leq k\leq |\mathcal{M}|} \{-c_{ik} - \rho_k\} - \epsilon \qquad \forall i \in \mathcal{C},\ j\ \text{s.t.}\  x^*_{ij}=1,
%		\label{eq:epsilonCS}
%	\end{equation}	 
%where $\rho_j=\max_{1\leq k\leq |\mathcal{C}|}\hat{B}(k,j)$ is the maximum bid among vehicles for customer $j$. This is called the $\epsilon-$complementary slackness ($\epsilon-$CS) condition. It can be shown that the auction algorithm terminates in finite time and the cost of assignment at termination is within $|\mathcal{C}|\epsilon$ of the optimal costs \cite{bertsekas1990auction}. 

%The auction algorithm lends itself to be easily solved in a distributed or parallel fashion \cite{bertsekas1990auction}. Zavlanos et al. \citep{zavlanos2008distributed} show that if the information of bid prices is shared between ``neighboring" vehicles, then a distributed version of the auction algorithm which updates the bid prices and assignment of each vehicle based on the bid prices and previous assignment of its neighbors can solve for system optimal even under restricted communication between vehicles. However, the proof of convergence assumes that the undirected graph connecting neighboring vehicles is fully connected. In ride sharing settings, all vehicles belong to the same company can be connected to each other; however, assuming that a vehicle of one company knows the bid prices of a vehicle of other company is not realistic as it ignores the constraints on information sharing.
%
%Naparstek and Leshem \cite{naparstek2014fully} present an alternate distributed implementation of the auction algorithm. In their structure, each vehicle maintains an estimate of the highest bid price for each customer and determines its bid prices based on that estimate. The estimate maintained by each vehicle is different and is updated only when a vehicle wins the bid on a certain customer. The proofs in \cite{naparstek2014fully} show that the distributed implementation terminates and converge to an assignment with costs within $|\mathcal{C}|\epsilon$ of the optimal costs.

In the next section, we demonstrate that the architecture of \Coop~protocol has several parallels with that of the distributed auction algorithm in \cite{naparstek2014fully} and use this similarity to prove the optimality of the \texttt{Cooperative} protocol.

%can be modeled using the same structure like the distributed auction algorithm in \cite{naparstek2014fully}.

%We argue that the bidding process in the \texttt{Cooperaitve}
%
%architecture in \citep{naparstek2014fully} is reasonable for ridesharing settings. Each vehicle of a company maintains an estimate of the highest bid price for each customer and updates that estimate only when any vehicle of the same company wins a bid over the same customer. If a vehicle of other company wins the bid, then the estimate is not updated. This distributed sharing of information mimics the real world where companies do not share information (about the location of their vehicles and the bid prices) with each other, but only learn to update their bids once the broker informs them if they did not win the bid. This distributed architecture is privacy-aware and is thus used in the \texttt{Cooperative} model. The only difference is that, to make the architecture more realistic, we redefine the bidders as the companies, instead of the vehicles. We explain the \texttt{Cooperative} model in the next section.

%If one wants to use the vocabulary used in the auction algorithm literature, this positions the vehicle as the bidder and the task as the act of picking up a customer. At each time step $t$, i.e. the end of a batch period, the vehicles bid to be assigned to customers in the pool of requests.

%The auction algorithm uses the idea that each customer $j\in \mathcal{M}$ has an associated cost $\rho_j$ which a vehicle will pay if the customer is assigned to the vehicle. Given a positive scalar $\epsilon$, an assignment $x_{ij}$, and price for each object $\rho_j$, a vehicle is defined as \emph{happy} with the assignment if its profit is within $\epsilon$ of the maximum achievable profit. 

%\Cmm{Define L$\epsilon-$CS condition}
%
%
%\Cmm{Talk about centralized vs distributed algorithms.}
%
%\Cmm{Say it is privacy-aware. }

%\begin{itemize}
	%\item \vpnote{Talk about the dual optimization problem in terms of prices}
	%\item \vpnote{Insert the standard auction algorithm}
	%\item \vpnote{In terms of proofs on performance guarantee: state the proof that maximum number of iterations is bounded by XX}
%\end{itemize}

%Assuming that all vehicles have access to price of each object is equivalent to assuming that a vehicle knows the bids of all other vehicles. This may be an unreasonable assumption for a multi-company setting. We now introduce two frameworks for assignment in the presence of multiple companies differentiated based on the level of cooperation between the companies.

%\subsection{The three models of ridesharing}
%
%We describe in detail the three models of interaction between multiple companies presented in Figure \ref{fig:framework}. In particular, in the scope of the paper, we will focus on the \texttt{Cooperative} and \texttt{Competitive} models. We have: 
%\begin{itemize}
%\item The \texttt{Centralized} model where a broker computes the costs associated with assigning each vehicle to any customer and seeks to find the optimal solution to the \textbf{LAP(}$C,\mathcal{M}$\textbf{)}. This can be solved using efficient and scalable algorithms, e.g. centralized auction algorithms~\cite{bertsekas1990auction}.
%
%%each vehicle shares its bid information with all other vehicles and a broker makes decisions for all customers. 
%\item The \texttt{Cooperative} model where the broker does not require access to the location of the vehicles, instead the broker interacts with each company by iteratively asking for the two best bid prices for the yet unassigned customers.{\vpnote{Comment: I think the bid price is still one, but it is evaluated as a difference between costs of two best customers for each company. Revise this based on updated discussion in Section 4.}} This model, which is essentially an extension of the distributed auction algorithm~\cite{naparstek2014fully}, runs until all customers are assigned to vehicles. It relies on a distributed architecture, and minimizes information sharing (no proprietary information of the companies is shared) but, as we shall prove, still enables to solve \textbf{LAP}$(\mathcal{C},\mathcal{M})$ to optimality. Extensions of this protocol are the \texttt{Cooperative with Stochasticity} model which aims to model the noise that can come from the vehicle positioning errors and the routing computations, and the \texttt{Cooperative with Stochasticity and Bias} model as the routing/map service may be different among the companies and a given routing service may provide consistently shorter/longer travel times compared to others. 
%%broker 
%%only the vehicles belonging to the same company share the bid information, but a broker still makes decisions for all customers by interacting with the vehicles and their bids. 
%\item The \texttt{Competitive} model where there is no broker to coordinate the assignment process, and customers send their requests to the company, for example through a broker application on their smartphone. Each company $p$ solves \textbf{LAP(}$C_p, \mathcal{M}$\textbf{)} and submit bid offers directly to customers $j$ with $x_{ij}=1, i \in  \mathcal{C}_p$. The customers who receive an offer then select the best offer among the companies and are considered assigned. Each company then resolves the assignment considering all unassigned customers. The process continues until all customers are assigned. An extension of this protocol is the \texttt{Competitive with Preference} model which models the fact that customers always choose the offer from the company they prefer.
%%In this protocol, 
%\end{itemize}

%\begin{multicols}{3}
%	%Use this to explain the three algorithms space permitting.
%	This is column 1
%	\columnbreak
%	
%	This is column 2
%	
%	\columnbreak
%	This is column 3
%
%\end{multicols}

%Our objective is to compare the performance of the information sharing settings in \texttt{Distributed} and \texttt{No-communication} protocols against the optimal performance of the \texttt{Centralized} protocol.




%Let $x_{ij} \in \{ 0,1\}, i \in \mathcal{C}, j \in \mathcal{M}$ be the set of binary variables: $x_{ij}=1$ only if vehicle $i$ is assigned to customer $j$, otherwise $x_{ij}=0$. We denote by $j_i$ the customer $j \in \mathcal{M}$ assigned to a vehicle $i \in \mathcal{C}$, that is, $x_{i,j_i}=1$. Let $c_{ij} \in \mathbb{R}_+$ denote the cost incurred by the vehicle if it is assigned to customer $j$. This cost is a function of different vehicle and customer parameters including detour time required to add the new customer to the current schedule, vehicle capacity, preference of customers already onboard etc. Let $\mathcal{I} : \mathcal{C} \times \mathcal{M} \rightarrow \mathbb{R}_+$ denote the cost function, where $\mathcal{I}(i,j)=c_{ij}$. We set $\mathcal{I}(i,j)= \infty$ if a vehicle $i$ cannot accommodate the request for customer $j$.


%In the presence of multiple companies, ensuring that the assignment is optimal is difficult.



==> abstract.tex <==
Ridesharing has been emerging as a new type of mobility. However, the early promises of ridesharing for alleviating congestion in cities may be undermined by a number of challenges, including the growing number of proposed services and the subsequent increasing number of vehicles, as a natural consequence of competition. In this work, we present optimization-based approaches to model cooperation and competition between multiple ridesharing companies, in a real-time on-demand setting. A recent trend relies on solving the integrated combination of Dial-A-Ride Problems (DARP), which compute the cost of assigning incoming requests to vehicle routes, plus Linear Assignment Problems (LAP), which assign vehicles to requests. While the DARPs, are solved at the level of the vehicles of each company, we introduce cooperative and competitive approaches to solve the LAP. The cooperative model, which could make use of Mobility as a Service platforms, is shown to solve the LAP to optimality following closely results from the literature, and limiting the amount of information the companies are required to share. We investigate how a realistic model of competition deviates from this optimality and provide worst case bounds. We evaluate these models with respect to a centralized model on one-week instances of the New York City taxi dataset. Model variants coping with noise in the travel time estimations, bias in the assignment costs, and preferences in the competitive case are also presented and validated. The computational results suggest that cooperation among ridesharing companies can be conducted in such a way to limit the degradation of the level of service with respect to a centralized model. Finally, we argue that the competition can lower the quality of the ridesharing service, especially in the case customer preferences are accommodated.
